KompaRe: A Knowledge Graph Comparative Reasoning System

Reasoning is a fundamental capability for harnessing valuable insight, knowledge and patterns from knowledge graphs. Existing work has primarily been focusing on point-wise reasoning, including search, link predication, entity prediction, subgraph matching and so on. This paper introduces comparative reasoning over knowledge graphs, which aims to infer the commonality and inconsistency with respect to multiple pieces of clues. We envision that the comparative reasoning will complement and expand the existing point-wise reasoning over knowledge graphs. In detail, we develop KompaRe, the first of its kind prototype system that provides comparative reasoning capability over large knowledge graphs. We present both the system architecture and its core algorithms, including knowledge segment extraction, pairwise reasoning and collective reasoning. Empirical evaluations demonstrate the efficacy of the proposed KompaRe.

==> 007relwork.tex <==
\section{Related Work}


{\bf A - Knowledge Graph Search.} Many efforts have been made for searching and browsing large knowledge graphs. 
Wang et al. ~\cite{Wang2015QUT} proposed a Bayesian probability model combined with random walks to find the most similar concepts for a given query entity.
Lei et al. ~\cite{lei2018} developed a system to answer natural language question over knowledge graphs, where the natural language question is transformed into a query graph and the question-answering thus becomes a subgraph matching problem. 
Wu et al. ~\cite{YinghuiWu} discovered that the background knowledge graph can be described by many small-sized patterns. 
%To speedup the graph searching process, 
They developed an effective mining algorithm to summarize the large knowledge graph according to small-sized patterns.
Yang et al. ~\cite{Yang2014vldb} found that due to the lack of insight about the background knowledge graph, it is often hard for a user to precisely formulate a query. They developed a user-friendly knowledge graph search engine to support query formation and transformation. 
Jayaram et al. ~\cite{GQBE} proposed a knowledge graph query system called {\em GQBE}. Different from other graph query systems, {\em GQBE} focuses on entity tuple query which consists of a list of entity tuples.
Zhang et al. ~\cite{tongtao2018Gaia} developed a comprehensive multi-modality knowledge extraction and hypothesis generation system which supports three types of queries, including (1) class-based queries %which aim to find all instances of a known class in the knowledge graph; (e.g. find all "politician") 
(2) zero-hop queries %which aim to find all instances of an entity; (e.g. find all entities with name "Barack Obama") 
and (3) graph-queries. % which aim to find a graph. 


\noindent {\bf B - Knowledge Graph Reasoning.} Generally speaking, there are two types of knowledge graph reasoning methods, including (1) embedding based approaches and (2) multi-hop approaches. For the former, 
the main idea is to learn a low dimensional vector for each entity and predicate in the embedding space, and use these embedding vectors as the input of the reasoning tasks (e.g.,~\cite{transE}, ~\cite{rotatE}, ~\cite{entity-predicate}, ~\cite{tensor}, ~\cite{pprop}).
For the latter, %\hh{1-2 sentenses on its key ideas and cite William cohen's random walk based method. William Wang's meta-reasoning method, etc.}
the main idea is to learn missing rules from a set of relational paths sampled from the knowledge graph (e.g.,~\cite{williamCohen}, ~\cite{willianWang}, ~\cite{das-etal-2017-chains}, ~\cite{neelakantan-etal-2015-compositional}). Many effective reasoning methods have been developed for predicting the missing relation (i.e., link prediction) or the missing entity (i.e., entity prediction). 
In link prediction, given the `subject' and the `object' of {\em a triple}, it predicts the existence and/or the type of relation. 
For example,
{\em TransE}~\cite{transE} learns the low dimensional embedding of both entities and predicates in the knowledge graph; %. The relationship between two entities can be predicated by the translation between the embeddings of entities.
{\em TransR}~\cite{Lin2015TransR} learns the embedding of entities and predicates in two separate spaces. 
The learned embedding (either by {\em TransE} or {\em TransR}) can be used for both link predication and entity predication. 
%In ~\cite{SimplE}, \lliu{xxxxxxxxxx}. 
In entity prediction, given the `subject' and the `predicate' of {\em a triple}, it predicts the missing `object'. For example, 
%\hh{a few representative work, 1-2 sentences for each of them} 
{\em GQEs}~\cite{entity-predicate} embeds the graph nodes in a low dimensional space, and treats the logical operators as learned geometric operations. Given a query graph with missing entities,  {\em GQEs} can effectively predict the missing entities in the query graph. 


In recent years, knowledge graph reasoning has demonstrated strong potential for computational fact checking. Given {\em a claim} in the form of a triple of the knowledge graph, it reasons whether the claim is authentic or falsified. For example, 
in ~\cite{Shiralkar2017}, the authors focused on checking the truthfulness of a given triple/claim, by first transforming the knowledge graph into a weighted directed graph, and then extracting a so-called knowledge stream based on maximum flow algorithm. %First, they transformed the knowledge graph into a line graph to model the co-occurrence of different predicates, and they used a TF-IDF method to calculate the similarity between different predicates. Then, they transferred the knowledge graph into a directed weighted graph and used a minimum cost maximum flow algorithm to find the knowledge stream between the give subject and object. If the truth score of the knowledge stream is too low, they thought that the query is false.
It is worth mentioning that the extracted knowledge stream can be viewed as an edge-specific knowledge segment in \gchecker. 
In ~\cite{Shi2016dpp}, an alternative method was developed to detect fake claims by learning the discriminative paths of specific predicates. Different from \cite{Shiralkar2017}, this is a supervised reasoning method since 
it requires different training data sets for different predicates. 
If the predicate in the claim does not exist in the training data, which is likely to be the case for detecting falsified claims in emerging news, the algorithm becomes inapplicable.
 As mentioned before, these methods belong to point-wise reasoning. Therefore, %Thus, although being effective in detecting a single falsified claim, 
 they might fall short in detecting the semantic inconsistency between multiple claims.

%However, all the above methods focus on fact checking for a single claim, link predication or entity predication , and thus is incapable of detecting the semantic inconsistencies between different claims.


\hide{

\begin{table*}[]
	\centering
	\caption{Summary of Existing KG Search and Comparative Reasoning Systems}
	\vspace{-0.5\baselineskip}
	\resizebox{\textwidth}{!}{
	\begin{tabular}{|c|c|c|c|}
		\hline
		Name & Input                                              & Output         &       KG Systems    \\ \hline
		\tt{F1} & A single query node                                & Top-{\em k} Entities  & ~\cite{Tong2006rdwalk} ~\cite{Lin2015TransR} ~\cite{Mikolov2013DRW} \\ \hline
		\tt{F1'} & A single query node                             & A subgraph with most relevant entities and edges w.r.t the query node & None \\ \hline
		\tt{F2} & A Single query edge                                & Knowledge segment & ~\cite{Shiralkar2017} ~\cite{Shi2016dpp} ~\cite{lei2018} \\ \hline
		\tt{F3} & Two or more query edges                        & commonality and inconsistency & None \\ \hline
		\tt{F4} & A query graph                               & A matching subgraph  & ~\cite{Su2015KDD} ~\cite{lei2018} ~\cite{Zou2011GAS} ~\cite{Yahya2016RQE} \\ \hline
		\tt{F4'} & A query graph                               & A semantic matching subgraph/Knowledge Segment  & None \\ \hline
		%~\cite{Faloutsos2004} ~\cite{Tong2006CSP} ~\cite{Su2015KDD} ~\cite{Tong2007FBP} ~\cite{lei2018} \\ \hline
		%multiple query nodes                               & \thead{Connection Pathways \\ for Marked Nodes} & ~\cite{Koren2006MEP} ~\cite{Tong2006CSP}  \\ \hline
		\tt{F5} & Multiple query nodes               & Grouping and connection pathways & None \\ \hline
		\tt{F6} & A single node/edge and multiple KG               & Commonality and differences in different KGs & None \\ \hline
		\end{tabular}
	}
\label{table:existing:kgsys}
\vspace{-0.8\baselineskip}
\end{table*}
}


%\hh{have u checked this tutorial? \url{https://sites.cs.ucsb.edu/~william/papers/Part3_KB_Reasoning.pdf}? seems that we have already consider these tasks, link prediction, entitiy prediction, fact checking. just make sure we do not miss important aspect of kg reason from existing work}
%\lliu{Hi professor, I have checked this tutorial before. I will add more work about kg reason here.}
%\hh{check this paper~\cite{Leman2013SIAM} -- some components of their system might be related to KG search and reasoning}

%In ~\cite{qi2018ICDE}, the authors proposed a graph summarization framework to facilitate knowledge graph search. They first summarize the knowledge graph into a concreate graph according to some frequent graph pattern, then they find the (approximate) answers according to the query. 
%\hh{a little bit more details, e.g., what is the main functions (in input/output format)?}
%In ~\cite{Su2015KDD}, they used the feedback information to enhance the knowledge graph query performance.
%In ~\cite{slq2014vldb}, they proposed a system SLQ.


==> _002probDef.tex <==
In this section, we formally give the definition of this paper. Table ~\ref{table1} gives the notations used in our paper.
A knowledge graph can be treated as set of triples $<Subject, Predicate, Object>$ ($<s, p, o>$ for short) where "Subject" and "Object" are the entities in the knowledge graph and "Predicate" are the relationship between two entities. If we treat the knowledge graph as an attributed graph, the entities will correspond to the nodes in the attributed graph, and predicates correspond to the attributed edges. So, We can also use $G=(V, E, L)$ to denote the knowledge graph where $V$ is the set of entities or nodes, $E$ is the set of predicates or edges and $L$ is the label set of nodes and edges. We will use both of these two definitions in our paper.


\begin{table}[]
	\centering
	\caption{Notations and Definition}
	\vspace{-0.5\baselineskip}
	\begin{tabular}{|c|l|}
		\hline
		Symbols       & Definition                \\ \hline
		$\mathcal{Q}$=\{$V_Q$, $E_Q$, $L_Q$\} & an attributed query graph \\ \hline
		$\mathcal{G}$=\{$V_G$, $E_G$, $L_G$\} & an attributed data graph  \\ \hline
		$\mathcal{H}_{i}$         & a partial matching with $i$ nodes \\ \hline
		$\mathcal{Q}_{i}$         & a partial query graph with $i$ nodes \\ \hline
		$u$, $\hat{u}$      & nodes in query graph      \\ \hline
		$v$, $\hat{v}$      & vertices in data graph       \\ \hline
		m($u_i$) = $v_i$ & matching function       \\ \hline
		N($u$)          & neighborhood of query node $u$  \\ \hline
		C($u$)          & candidate set of query node $u$  \\ \hline
		f($\mathcal{Q}$, $\mathcal{H}$)          & the loss function     \\ \hline
	\end{tabular}
\label{table1}
\vspace{-0.8\baselineskip}
\end{table}

==> _002probDef01match.tex <==


Knowledge graph searching or graph querying in knowledge graph has been studied for a long time. 
The knowledge graph searching mainly focus on given a query graph, query pattern or SPARQL query which specified by users based on their own knowledge, finding a matching subgraph in the underlying knowledge graph, or given a NLP query, constructing a corresponding query graph and finding the matching subgraphs. 
In this paper, the query can be a node, and edge or a semantic query graph. The definition of the semantic query graph is given below.

\begin{definition}{Semantic Query Graph}
The semantic query graph can be denoted as $Q=(V, E)$ where $V$ is the set of entities in the query graph, and $E$ is the set of predicates in the query graph.
\end{definition}

Also different traditional knowledge graph searching algorithm, Given a semantic query graph $Q$, we hope to find a knowledge segment for the query graph. More specifically speaking, for each triple in the query graph $Q$, We will reason over the underlying knowledge graph to extract a semantic connection subgraph from it, with the subject and object nodes as the source and target nodes. We call the result as knowledge segment which is defined as below.

\begin{definition}{Knowledge Segment/Semantic subgraph}
Give a knowledge graph $G$ and semantic query $Q$, the knowledge segment can be denoted as $KS_Q = (V, E)$ which satisfies that $V_Q \in V_K$ and for each $e \in E_Q$, it has a correspond subgraph $G_s$. And $KS_Q = \cup G_s$.
\end{definition}


The main function of our system for knowledge graph searching can be divided into three parts: (1) given a node, finding its corresponding entity in the knowledge graph \textbf{G}; (2) given a edge, finding its corresponding knowledge Segment in the knowledge graph; (3) given a semantic subgraph \textbf{Q}, finding its corresponding knowledge segment in the knowledge graph.

%\lliu{Hi professor Tong, According to the results returned by Google, knowledge graph reasoning can be divided into 4 parts: missing entity predication, missing link predication, rules learning and fact prediction (Given a triple, predict whether it is true or fale).} 
%\hh{good, summarize these tasks in Table 2}

%\lliu{This is the definition from paper "A review: Knowledge reasoning over knowledge graph".  Knowledge reasoning over knowledge graphs aims to identify errors and infer new conclusions from existing data. New relations among entities can be derived through knowledge reasoning and can feed back to enrich the knowledge graphs, and then support the advanced applications. }

In summary, we could define our subgraph searching problem as below.


\begin{pro-stat}{Knowledge Graph Searching}
	
	\textbf{Given:} (1) A underlying knowledge graph; (2) A single node, a single edge or a semantic query graph.
	
	\textbf{Find:} (1) A list of node; (2) A Knowledge Segment.
	
\end{pro-stat}



==> _002probDef02Reason.tex <==



Knowledge graph reasoning has been studied for a long time, the goal of knowledge graph reasoning is to discover new knowledge or detect errors from the existing data. Currently, the application of knowledge graph reasoing can be divided into 4 parts: missing entity predication, missing link predication, rules learning and fact prediction (Given a triple, predict whether it is true or fale). Different from these methods, in our system, we focuses on knowledge graph comparative reasoning. More specifically speaking, given multiple piece of information the user has (multiple query nodes/edges/subgraphs), we aim to find their commonality (the intersection/AND), the difference (the diff) and the union. Or given the same input, but multiple KGs, we will compare and reason the search results from different KGs. Comparative knowledge graph reasoning has a lot of applications. One of the most useful application is detecting the fack news.

The idea behind comparative reasoning is that if two knowledge segments are common. They should have high similarity. If there are some inconsistencies, after we alter the inconsistent elements which could be node, edge and/or attributes, the similarity between these two knowledge segments could significantly improved.
Formally, the problem can be defined as below.
\begin{definition}{Comparative knowledge graph reasoning:}
Given two knowledge segements $KS_1$ and $KS_2$, found the common node set $VS$ and edge set $ES$ which satisfy $(VS, ES) = KS_1 \cap KS_2$. and find the elements that could significantly improve the similarity between two knowledge segments.
\end{definition}







%\hh{some additional functions we can consider (we might not implement them in this version of the system): (1) sense-making (given multiple query nodes, find groups between them, and for each group, find the best connection within the group ~\cite{Leman2013SIAM}, (2) given a single node/edge and multiple KGs, find commonality and differences in different KGs}





%\hh{let us try to have a table to summarize the different functions and whether any existing system and/or our system support it: first column: input; second column: output: third column: system XYZ~\cite{}, our method, etc. this will help differentiate our system to the existing works and also guide us which functions we should put more emphasis on}


%\hh{we can discuss this more -- one possible distinctive feature that differentiate us from the existing work might be the reasoning/comparison capability of our system. the existing work mostly focus on finding things that the user wants (given a query graph or spark query, find a match; given a NLP query, construct  the corresponding query graph. in contrast, in our system, given multiple piece of information the user has (multiple query nodes/edges/subgraphs, we will be able to find their commonality (the intersection/AND), the difference (the diff) and the union. or given the same input, but multiple KGs, we will compare and reason the search results from different KGs}








==> _004search.tex <==





%\subsubsection{Predicate Entropy Random Walk With Restart}


%\subsubsection{Nibble on knowledge graph}

%Besides finding the most relevant entities w.r.t. the query entity, sometimes we may prefer to find a subgraph around the query entity. Compared with high similarity but disconnected entities, a connected subgraph may reveal more information about the entity. To achieve this goal, we generalize Nibble-PageRank ~\cite{nibble} to knowledge graph. 
%Nibble-PageRank is a local graph partitioning algorithm which is used to find dense cluster in the graph. 
%When generalize Nibble-PageRank to knowledge graph, we first transform the knowledge graph to a weighted graph according to the predicate entropy, then we use Nibble-PageRank to find the connected subgraph around the query entity.











==> theme/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering
